The featureless and non-variable optical spectral energy distribution of AXP 4U 0142+61

We present GTC-10.4m spectroscopy and multi-band photometry of the faint (r ~26) optical counterpart of the anomalous X-ray pulsar 4U 0142+61. The 5000 - 9000 Angs spectrum -- the first obtained for a magnetar -- is featureless, allowing us to set an equivalent width upper limit EW < 25 Angs to the presence of emission lines in the Halfa region. Multi-band photometry in the g, r, i, z SDSS bands obtained at different epochs over 12 years shows no significant variability from minutes-to-years time scales. The photometry has been calibrated, for the first time, against the SDSS itself, resulting in solid upper limits to variability ranging from ~0.2 mag in i (over 12 years) to 0.05 mag in z (over 1.5 years). The shape of the optical + near-infrared (literature values) spectral energy distribution is not well constrained due to the high extinction along the line of sight. Using a Markov Chain Monte Carlo analysis we find that it can be described by a power-law with a spectral index beta=-0.7+-0.5 and E_(B-V)=1.5+-0.4. We also discuss on the implications of adding hard X-ray flux values from literature to the spectral fitting.

==> def_bibtex.tex <==
\def\apj{ApJ}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\apjl{ApJ}
\def\pasj{PASJ}
\def\nat{Nature}
\def\iaucirc{IAU Circ.}
\def\skytel{S\&T}
\def\aaps{A\&A S.S.}
\def\apss{Ap\&SS}
\def\apjs{ApJS}
\def\araa{ARA\&A}
\def\pasp{PASP}
